Regret-Optimal Defense Against Stealthy Adversaries: A System Level Approach

Modern control designs in robotics, aerospace, and cyber-physical systems rely heavily on real-world data obtained through system outputs. However, these outputs can be compromised by system faults and malicious attacks, distorting critical system information needed for secure and reliable operation. In this paper, we introduce a novel regret-optimal control framework for designing controllers that make a linear system robust against stealthy attacks, including both sensor and actuator attacks. Specifically, we present (a) a convex optimization-based system metric to quantify the regret under the worst-case stealthy attack (the difference between actual performance and optimal performance with hindsight of the attack), which adapts and improves upon the $\mathcal{H}_2$ and $\mathcal{H}_{\infty}$ norms in the presence of stealthy adversaries, (b) an optimization problem for minimizing the regret of (a) in system-level parameterization, enabling localized and distributed implementation in large-scale systems, and (c) a rank-constrained optimization problem equivalent to the optimization of (b), which can be solved using convex rank minimization methods. We also present numerical simulations that demonstrate the effectiveness of our proposed framework.

==> archive/sections/1_abstract.tex <==
\begin{abstract}
\begin{itemize}
    \item Dynamic regret optimal stealthy attack, less conservative objective than H infinity
    \item Thanks to SLS, it Leads to an almost SDP formulation
    \item We could also consider sensor attacks because now $\mathbf{y}$ is linear in $\mathbf{x}$ and $\mathbf{u}$
    \item Then, we can easily combine this with data using data-driven SLS
    \item The same convex relaxation approach as in the ZDA paper can be used here
    \item SLS can be distributed and localized
    \item SLS parameterized stabilizing controller?
    \item detectability of Bullo's paper in SLS language (as in controllability and observability)
\end{itemize}
\end{abstract}
%\begin{keywords}
%Robust control, Autonomous systems, and Machine learning.
%\end{keywords}
% Our main contribution is to enhance the performance of the learned motion planning policy with collision avoidance and tracking-based robustness guarantees, independently of its original performance such as approximation errors and regret bounds in machine learning.

==> archive/sections/2_introduction.tex <==
\section{Introduction}
\label{sec_introduction}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begin{itemize}
    \item Dynamic regret optimal stealthy attack <- less conservative objective than H infinity
    \item Thanks to SLS, it Leads to an almost SDP formulation
    \item We could also consider sensor attacks because now $\mathbf{y}$ is linear in $\mathbf{x}$ and $\mathbf{u}$
    \item Then, we can easily combine this with data using data-driven SLS
    \item The same convex relaxation approach as in the ZDA paper can be used here
    \item SLS can be distributed and localized
    \item SLS parameterized stabilizing controller?
    \item Deemphasize topology switching for this paper
\end{itemize}

==> archive/sections/3_preliminaries.tex <==
\section{Preliminaries and Problem Formulation}
\label{sec_preliminaries}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
In this paper, we consider the following discrete-time, networked linear control system:
\begin{subequations}
\label{eq_system}
\begin{align}
    x_{k+1} &= A_kx_k +B_{u,k}u(y_k,\nu_k)+B_{a,k}a_k\label{eq_continuous_initialx}\textcolor{white}{\eqref{eq_continuous_initialx}}\\
    y_k &= C_{y,k}x_k+D_{ya,k}a_k\label{eq_continuous_initialy}\textcolor{white}{\eqref{eq_continuous_initialy}}\\
    z_k &= C_{z,k}x_k+D_{zu,k}u_k\label{eq_continuous_initialz}\textcolor{white}{\eqref{eq_continuous_initialz}}
\end{align}
\end{subequations}
where $\nu_k$ is the topology representation of the network (\eg{}, adjacency matrix), $x_k$ is the stacked system state, $u$ is the stacked system control input, $a_k$ is the stacked attack control input, $y_k$ is the stacked system measurement, $z_k$ is the stacked regulated output for quantifying the control performance. As in~\cite{sls_ARC}, we use the following notations for the system signals: $\mathbf{x} = [x_0^{\top},\cdots,x_{T}^{\top}]^{\top}$, $\mathbf{u} = [u_0^{\top},\cdots,u_{T}^{\top}]^{\top}$, $\mathbf{a} = [x_0^{\top},a_0^{\top}\cdots,a_{T-1}^{\top}]^{\top}$, $\mathbf{y} = [y_0^{\top},\cdots,y_{T}^{\top}]^{\top}$, and $\mathbf{z} = [z_0^{\top},\cdots,z_{T}^{\top}]^{\top}$, where $u_k = u(y_k,\nu_k)$ and $T$ is the time horizon. We also use the following notations for the system matrices: $\mathcal{A} = \blkdiag(A_0,\cdots,A_{T-1},\mathbb{O})$, $\mathcal{B}_u = \blkdiag(B_{u,0},\cdots,B_{u,T-1},\mathbb{O})$, $\mathcal{B}_a = \blkdiag(\mathbb{I},B_{a,0},\cdots,\allowbreak B_{a,T-1})$, $\mathcal{C}_{{p}} = \blkdiag(C_{{p},0},\cdots,C_{{p},T})$, and $\mathcal{D}_{{p}{q}} = \blkdiag(\allowbreak D_{{p}{q},0},\cdots,D_{{p}{q},T})$, where ${q} \in \{u,a\}$ and ${p} \in \{y,z\}$. Then the system~\eqref{eq_system} can be written as
\begin{subequations}
\label{eq_system_bf}
\begin{align}
    \mathbf{x} &= \mathcal{Z}\mathcal{A}\mathbf{x}+\mathcal{Z}\mathcal{B}_{u}\mathbf{u}+\mathcal{B}_{a}\mathbf{a}\label{eq_system_bf_x}\textcolor{white}{\eqref{eq_system_bf_x}} \\
    \mathbf{y} &= \mathcal{C}_{y}\mathbf{x}+\mathcal{D}_{ya}\mathbf{a}\label{eq_system_bf_y}\textcolor{white}{\eqref{eq_system_bf_y}} \\
    \mathbf{z} &= \mathcal{C}_{z}\mathbf{x}+\mathcal{D}_{zu}\mathbf{u}\label{eq_system_bf_z}\textcolor{white}{\eqref{eq_system_bf_z}}
\end{align}    
\end{subequations}
where $\mathcal{Z}$ is the block-downshift operator, \ie{}, a matrix with identity matrices along its first block sub-diagonal and zeros elsewhere.

Throughout this paper, we consider the following output feedback control, which depends on the network topology $\bm{\nu} = (\nu_0,\cdots,\nu_T)$:
\begin{align}
    \label{eq_output_feedback}
    \mathbf{u} = \mathbf{K}(\bm{\nu})\mathbf{y}
\end{align}
which includes the feedback control with state estimation~\cite{sls_output_feedback_control} given as
\begin{align}
    \xi_{k+1} = A_{e,k}\xi_k+B_{e,k}y_k,~u_k = C_{e,k}\xi_k+D_{e,k}y_k
\end{align}
where $\xi_k$ is the internal state of the controller.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{System Level Parameterization}
\label{sec_sls}
Applying the feedback control of~\eqref{eq_output_feedback}, we get
\begin{align}
    \label{eq_system_with_feedback}
    \begin{bmatrix}
        \mathbf{x} \\
        \mathbf{u}
    \end{bmatrix}
    &=
    \begin{bmatrix}
        \mathbf{R} & \mathbf{R}\mathcal{Z}\mathcal{B}_{u}\mathbf{K} \\
        \mathbf{K}\mathcal{C}_y\mathbf{R} & \mathbf{K}+\mathbf{K}\mathcal{C}_y\mathbf{R}\mathcal{Z}\mathcal{B}_u\mathbf{K}
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf{{d}_x} \\
        \mathbf{{d}_y}
    \end{bmatrix} \\
    \mathbf{R} &= (\mathbb{I}-\mathcal{Z}\mathcal{A}-\mathcal{Z}\mathcal{B}_u\mathbf{K}\mathcal{C}_y)^{-1}
\end{align}
where $\mathbf{{d}_x} = \mathcal{B}_{a}\mathbf{a}$ and $\mathbf{{d}_y} = \mathcal{D}_{ya}\mathbf{a}$ denote the disturbance on the state and the measurement, respectively. If we simply write the system responses as 
\begin{align}
    \label{eq_sls_parameterization}
    \begin{bmatrix}
        \mathbf{x} \\
        \mathbf{u}
    \end{bmatrix}
    = 
    \begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    \mathbf{{d}}
    = 
    \begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    \begin{bmatrix}
        \mathbf{{d}_x} \\
        \mathbf{{d}_y}
    \end{bmatrix}
\end{align}
where $\mathbf{d}=[\mathbf{d_x}^{\top},\mathbf{d_y}^{\top}]^{\top}$, it can be verified that they satisfy the following affine relations due to~\eqref{eq_system_with_feedback}: 
\begin{subequations}
\label{eq_sls_conditions}
\begin{align}
    \label{eq_sls1}
    &\begin{bmatrix}
        \mathbb{I}-\mathcal{Z}\mathcal{A} & -\mathcal{Z}\mathcal{B}_u
    \end{bmatrix} 
    \begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathbb{I} & \mathbb{O}
    \end{bmatrix} \\
    \label{eq_sls2}
    &\begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    \begin{bmatrix}
        \mathbb{I}-\mathcal{Z}\mathcal{A} \\
        -\mathcal{C}_y
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathbb{I} \\
        \mathbb{O}
    \end{bmatrix}.
\end{align}
\end{subequations}
The conditions~\eqref{eq_sls1} and~\eqref{eq_sls2} are not just necessary but also \textit{sufficient} to ensure the existence of the output feedback controller, which allows us to directly work with the system level parameterization of~\eqref{eq_sls_parameterization}~\cite{sls_output_feedback_control,sls_tutorial,sls_tutorial}.
\begin{lemma}
\label{lemma_sls}
The affine subspace defined by~\eqref{eq_sls_conditions} parameterizes all possible system responses~\eqref{eq_sls_parameterization} achievable by the output feedback control~\eqref{eq_output_feedback}. Furthermore, for any matrices $(\mathbf{R},\mathbf{M},\mathbf{N},\mathbf{L})$ satisfying~\eqref{eq_sls_conditions}, the feedback control~\eqref{eq_output_feedback} with $\mathbf{K} = \mathbf
{L}-\mathbf{M}\mathbf{R}^{-1}\mathbf{N}$ achieves the desired response~\eqref{eq_system_with_feedback}.
\end{lemma}
\begin{proof}
The first part can be shown just by verifying~\eqref{eq_sls_conditions} for $(\mathbf{R},\mathbf{M},\mathbf{N},\mathbf{L})$ of~\eqref{eq_system_with_feedback}. The second part follows from substituting $\mathbf{K} = \mathbf
{L}-\mathbf{M}\mathbf{R}^{-1}\mathbf{N}$ into~\eqref{eq_system_bf} with the conditions of~\eqref{eq_sls_conditions}, which results in~\eqref{eq_sls_parameterization}. See~\cite{sls_output_feedback_control,sls_tutorial,sls_tutorial} for details.
\end{proof}

Thanks to Lemma~\ref{lemma_sls}, we can directly work with the system level parameterization~\eqref{eq_sls_parameterization} and the affine conditions to look for a controller~\eqref{eq_output_feedback} with a desired property. It also enables localized and distributed control implementation, which is suitable for large-scale networked control systems in this paper.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Regret Optimal Control}
Let $J(\mathbf{u},\mathbf{a})$ be some performance objective to be minimized, for the control and attack input defined in~\eqref{eq_system_bf}. The dynamic regret of $J$, which is the true optimal performance minus the optimal performance in hindsight, is defined as follows:
\begin{align}
    \label{eq_Jdefinition}
    \regret_{J}(\mathbf{u},\mathbf{a}) = J(\mathbf{u},\mathbf{a})-J^*(\mathbf{a}),~J^*(\mathbf{a}) = J(\mathbf{u_{nc}}(\mathbf{a}),\mathbf{a})
\end{align}
where $\mathbf{u}_{nc}$ is the optimal non-causal control policy, \ie{}, the optimal policy with the full knowledge of the past, current, and future attack histories $\mathbf{a}$.

Regret optimal control is for designing a control policy that minimizes the worst-case regret $\regret_{J}^{*}(\mathbf{u})$~\cite{regret_optimal_control,slsregret}, \ie{},
\begin{align}
    \label{eq_regret_policy}
    \mathbf{u}^{*} = \mathrm{arg}\min_{\mathbf{u}}\regret_{J}^*(\mathbf{u}),~\regret_{J}^*(\mathbf{u}) = \max_{\|\mathbf{a}\| \leq 1}\regret_{J}(\mathbf{u},\mathbf{a})~~~
\end{align}
This metric is shown to elegantly and adaptively interpolate 1) the robust performance of $\mathcal{H}_{\infty}$, which can be conservative as it considers only the worst-case performance, and 2) the average performance of $\mathcal{H}_2$, which can be too optimistic under the presence of adversarial disturbances~\cite{regret_original,regret_optimal_control}. It has also been shown recently in~\cite{slsregret} that regret optimal control works nicely with the system level parameterization of Sec.~\ref{sec_sls}.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Problem Formulation}
In this paper, we consider the following broad type of stealthy attack, which we call an $\alpha$-stealthy attack, where the corresponding system measurement can be non-zero as long as it is below a certain threshold.
%%%
\begin{definition}
\label{def_alpha_stealth}
For a given time horizon $T$, an attack $\mathbf{a}$ of~\eqref{eq_system_bf_x} is $\alpha$-stealthy in $k=1,\cdots,T$ if $\exists\alpha\in\mathbb{R}_{+}$ \st{} $\|\mathbf{y}-\mathbf{y_{n}}\|^2 \leq \alpha$, where $\mathbf{y}$ is given by~\eqref{eq_system_bf_y} and $\mathbf{y_{n}}$ is by $\mathbf{y}$ of~\eqref{eq_system_bf_y} with $\mathbf{a}=0$.
\end{definition}
%%%

The problems of our interest, in designing a general defense strategy against the $\alpha$-stealthy network adversaries, are summarized in the following.
\begin{enumerate}[label={\color{uiucblue}{(\alph*)}}]
    \item The regret optimal control~\eqref{eq_regret_policy} considers the worst-case regret for $\|\mathbf{a}\| \leq 1$. How can we derive a metric for the worst-case regret over the $\alpha$-stealthy attacks of Definition~\ref{def_alpha_stealth}, instead of $\|\mathbf{a}\| \leq 1$ (see Theorem~\ref{thm_regret_metric})?\label{item_problem1}
    \item How can we formulate the problem of finding the controller that minimizes the metric of~\ref{item_problem1}, with the system level parameterization for localized and distributed implementation in large-scale networks (see Proposition~\ref{proposition_sls_rstealthy_regret})? \label{item_problem2}
    \item How can we solve the problem~\ref{item_problem2} for the network topology $\bm{\nu}$ of~\eqref{eq_output_feedback} in a computationally tractable manner, so we can optimally detect and attenuate the $\alpha$-stealthy attacks (see Theorem~\ref{thm_convex_rank_constraint})?\label{item_problem3}
\end{enumerate}

==> archive/sections/4_regret.tex <==
\section{Regret Optimal Defense Against Stealthy Attacks}
\label{sec_regret}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
Consistently with the problem statement~\ref{item_problem1}, let us consider the following optimization problem for measuring the worst-case regret under the $\alpha$-stealthy attacks of Definition~\ref{def_alpha_stealth}:
\begin{align}
    \label{eq_regret_optimal}
    \sigma(\mathbf{u}) = \max_{\mathbf{a}}\regret_{J}(\mathbf{u},\mathbf{a})~\mathrm{\st{}}~\text{$\mathbf{a}$ is $\alpha$ stealthy}.
\end{align}
This metric allows us to consider the regret-based robustness simultaneously with the stealthiness of the attacks $a_k$ of~\eqref{eq_continuous_initialx}, as in the output-to-output gain derived for the $\mathcal{H}_{\infty}$-based robustness~\cite{outputL2gain}.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Optimal Non-Causal Control}
Defining the performance objective $J(\mathbf{u},\mathbf{a})$ of~\eqref{eq_Jdefinition} as $J(\mathbf{u},\mathbf{a}) = \|\mathbf{z}\|^2$, where $\mathbf{z}$ is the regulated output for the control performance given in~\eqref{eq_system_bf_z}, the non-causal optimal performance $J^*(\mathbf{a})$ of~\eqref{eq_Jdefinition} can be expressed as follows:
\begin{align}
    \label{eq_Jstar}
    J^*(\mathbf{a}) = \mathcal{J}(\mathbf{d}) = \min_{\mathbf{u}}\|\mathcal{E}\mathbf{u}+\mathcal{F}\mathcal{B}_a\mathbf{a}\|^2
\end{align}
where $\mathcal{E} = \mathcal{C}_z(\mathbb{I}-\mathcal{Z}\mathcal{A})^{-1}\mathcal{Z}\mathcal{B}_u+\mathcal{D}_{zu}$, $\mathcal{F} = \mathcal{C}_z(\mathbb{I}-\mathcal{Z}\mathcal{A})^{-1}$, and $\mathbf{d}=[\mathbf{d_x}^{\top},\mathbf{d_y}^{\top}]^{\top}$ for $\mathbf{d_x}$ and $\mathbf{d_y}$ of~\eqref{eq_sls_parameterization}. This problem is clearly convex and can be solved as~\cite{regret_optimal_control,slsregret} 
\begin{align}
    \label{eq_Q_nc_def}
    J^*(\mathbf{a}) =& \mathcal{J}^*(\mathbf{d}) = \|(-\mathcal{E}(\mathcal{E}^{\top}\mathcal{E})^{\dag}\mathcal{E}^{\top}+\mathbb{I})\mathcal{F}\mathbf{d_x}\|^2 = \mathbf{d}^{\top}\mathcal{Q}\mathbf{d} \\
    \mathbf{u_{nc}}(\mathbf{a}) =& -(\mathcal{E}^{\top}\mathcal{E})^{\dag}\mathcal{E}^{\top}\mathcal{F}\mathcal{B}_a\mathbf{a}
\end{align}
where $\dag$ denotes the pseudoinverse and $\mathcal{Q}$ is defined appropriately with these notations.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{System Level Approach to Worst-Case Stealthy Attack}
Let $\mathbf{\Omega} = (\mathbf{R},\mathbf{N},\mathbf{M},\mathbf{L})$ for the system level parameterization~\eqref{eq_sls_parameterization}. Then the constraint of~\eqref{eq_regret_optimal} can be written as
\begin{align}
    \label{eq_stealth_con}
    &\mathbf{d}^{\top}\Phi(\mathbf{\Omega})^{\top}\Phi(\mathbf{\Omega})\mathbf{d} \leq \alpha,~\Phi(\mathbf{\Omega})
    =
    \begin{bmatrix}
        \mathcal{C}_y\mathbf{R} & \mathcal{C}_y\mathbf{N}+\mathbb{I}
    \end{bmatrix}
\end{align}
by Definition~\ref{def_alpha_stealth}. Also, $J(\mathbf{u},\mathbf{a}) = \mathcal{J}(\mathbf{\Omega},\mathbf{d}) = \|\mathbf{z}\|^2$ of~\eqref{eq_Jdefinition} with $\mathbf{z}$ of~\eqref{eq_system_bf_z} is given as
\begin{align}
    \label{eq_stealth_obj}
    \mathcal{J}(\mathbf{\Omega},\mathbf{d}) &= 
    \mathbf{d}^{\top}
    \Psi(\mathbf{\Omega})^{\top}
    \Psi(\mathbf{\Omega})
    \mathbf{d} \\
    \Psi(\mathbf{\Omega})
    &=
    \begin{bmatrix}
        \mathcal{C}_z\mathbf{R}+\mathcal{D}_{zu}\mathbf{M} & \mathcal{C}_z\mathbf{N}+\mathcal{D}_{zu}\mathbf{L}
    \end{bmatrix}
\end{align}
The metric~\eqref{eq_regret_optimal} thus becomes the following quadratically constrained quadratic program (QCQP), expressed in therms of the system level parameterization of~\eqref{eq_sls_parameterization}:
\begin{align}
    \label{eq_stealth_qcqp}
    \varsigma(\mathbf{\Omega}) = \max_{\mathbf{d}}\mathbf{d}^{\top}(
    \Psi^{\top}
    \Psi-\mathcal{Q})
    \mathbf{d}~\mathrm{\st{}}~\mathbf{d}^{\top}\Phi^{\top}\Phi\mathbf{d} \leq \alpha
\end{align}
where the argument $\mathbf{\Omega}$ for $\Phi$ and $\Psi$ are omitted for notational simplicity, and $\mathcal{Q}$, $\Phi$, and $\Psi$ are given in~\eqref{eq_Q_nc_def}, \eqref{eq_stealth_con}, and~\eqref{eq_stealth_obj}, respectively. QCQPs are known to enjoy strong duality if Slater's condition holds~\cite[pp. 653-658]{citeulike:163662},\cite{slsregret}, which leads to the following theorem.
\begin{theorem}
\label{thm_regret_metric}
The QCQP for the regret optimal metric for $\alpha$-stealthy attacks~\eqref{eq_stealth_qcqp} is equivalent to the following convex optimization problem:
\begin{align}
    \label{eq_regret_metric_convex}
    \mu(\mathbf{\Omega}) = \min_{\lambda\geq 0}\lambda\alpha~\mathrm{\st{}}~\lambda\Phi(\mathbf{\Omega})^{\top}\Phi(\mathbf{\Omega})-\Psi(\mathbf{\Omega})^{\top}\Psi(\mathbf{\Omega})+\mathcal{Q} \succeq 0~~~
\end{align}
and thus $\mu(\mathbf{\Omega}) = \varsigma(\Omega)$ for $\varsigma$ of~\eqref{eq_stealth_qcqp}.
\end{theorem}
\begin{proof}
The Lagrangian of the QCQP~\eqref{eq_stealth_qcqp} is given as follows:
\begin{align}
    L(\mathbf{d},\lambda) = \lambda(\mathbf{d}^{\top}\Phi^{\top}\Phi\mathbf{d}-\alpha)+\mathbf{d}^{\top}(-\Psi^{\top}\Psi+\mathcal{Q})\mathbf{d}
\end{align}
which gives the Lagrange dual function $g(\lambda)$ defined as
\begin{align}
    g(\lambda) = \min_{\mathbf{d}}L
    =
    \begin{cases}
    -\lambda\alpha & \text{$\lambda\Phi^{\top}\Phi-\Psi^{\top}\Psi+\mathcal{Q} \succeq 0$}\\
    -\infty & \text{otherwise}
    \end{cases}.
\end{align}
As a result, we get the following convex optimization problem:
\begin{align}
    \min_{\lambda\geq 0}\lambda\alpha~\mathrm{\st{}}~\lambda\Phi^{\top}\Phi-\Psi^{\top}\Psi+\mathcal{Q} \succeq 0.
\end{align}
Since the original QCQP~\eqref{eq_stealth_qcqp} is strictly feasible for $\mathbf{d} = 0$ when $\alpha\in\mathbb{R}_{+}$, strong duality holds~\cite[pp. 653-658]{citeulike:163662}.
\end{proof}

Again, the metric~\eqref{eq_regret_metric_convex} provides a novel approach for quantifying the worst-case regret for controllers with the system level parameterization of Sec.~\ref{sec_sls}. As discussed for the case of the output-to-output gain in~\cite{outputL2gain}, this metric can be viewed as one of the system gains from the $\alpha$-stealthy attack $\mathbf{a}$ of~\eqref{eq_system_bf_x} to the regret of the regulated performance output $\mathbf{z}$~\eqref{eq_system_bf_z}, which gives our answer to the problem~\ref{item_problem1}. Theorem~\ref{thm_regret_metric} thereby establishes an alternative but more sophisticated measure to evaluate the systems' resilience against stealthy attacks via convex optimization, adaptively with the use of the regret, in lieu of the conventional system gains including $\mathcal{H}_{\infty}$ and $\mathcal{H}_2$.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Regret Optimal Defense via Topology Switching}
We are now ready to design a feedback control policy in terms of the system level parameterization of Sec.~\ref{sec_sls}, which minimizes the novel metric $\mu$ of~\eqref{eq_regret_metric_convex} in Theorem~\ref{thm_regret_metric} for regret optimal stealthy attack attenuation.
\begin{proposition}
\label{proposition_sls_rstealthy_regret}
Consider the following optimization problem in terms of the system level parameterization $\mathbf{\Omega} = (\mathbf{R},\mathbf{M},\mathbf{N},\mathbf{L})$ of~\eqref{eq_sls_parameterization}:
\begin{subequations}
\label{eq_prop_nonconvex}
\begin{align}
    &\mu^* = \min_{\mathbf{\Omega},\lambda}\lambda\alpha\label{eq_obj_prop}\textcolor{white}{\eqref{eq_obj_prop}} \\
    &\mathrm{\st{}}~\lambda\Phi(\mathbf{\Omega})^{\top}\Phi(\mathbf{\Omega})-\Psi(\mathbf{\Omega})^{\top}\Psi(\mathbf{\Omega})+\mathcal{Q} \succeq 0\label{eq_con_prop}\textcolor{white}{\eqref{eq_con_prop}} \\
    &\textcolor{white}{\mathrm{\st{}}~}
    \begin{bmatrix}
        \mathbb{I}-\mathcal{Z}\mathcal{A} & -\mathcal{Z}\mathcal{B}_u
    \end{bmatrix} 
    \begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathbb{I} & \mathbb{O}
    \end{bmatrix} \label{eq_sls1_prop}\textcolor{white}{\eqref{eq_sls1_prop}} \\
    &\textcolor{white}{\mathrm{\st{}}~}
    \begin{bmatrix}
        \mathbf{R} & \mathbf{N} \\
        \mathbf{M} & \mathbf{L}
    \end{bmatrix}
    \begin{bmatrix}
        \mathbb{I}-\mathcal{Z}\mathcal{A} \\
        -\mathcal{C}_y
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathbb{I} \\
        \mathbb{O}
    \end{bmatrix} \label{eq_sls2_prop}\textcolor{white}{\eqref{eq_sls2_prop}}\\
    &\textcolor{white}{\mathrm{\st{}}~}\mathbf{\Omega} \in \mathfrak{S} (= \mathrm{set~for~system~level~constraints)},~\lambda\geq0\label{eq_sls3_prop}\textcolor{white}{\eqref{eq_sls3_prop}}
\end{align}
\end{subequations}
where $\mathcal{Q}$, $\Phi$, and $\Psi$ are given in~\eqref{eq_Q_nc_def}, \eqref{eq_stealth_con}, and~\eqref{eq_stealth_obj}, respectively, and the other notations are given in~\eqref{eq_system_bf}.
The output feedback control of~\eqref{eq_output_feedback} with $\mathbf{K} = \mathbf{K}^* = \mathbf
{L}^*-\mathbf{M}^*{\mathbf{R}^*}^{-1}\mathbf{N}^*$ achieves the desired response~\eqref{eq_system_with_feedback} and the regret optimal resilience against $\alpha$-stealthy attacks of Definition~\ref{def_alpha_stealth}, where $\mathbf{\Omega}^* = (\mathbf{R}^*,\mathbf{M}^*,\mathbf{N}^*,\mathbf{L}^*)$ is the optimizer of~\eqref{eq_prop_nonconvex}. In particular, for the dynamic regret given as $\regret_{\mathcal{J}}(\mathbf{\Omega},\mathbf{d}) = \mathcal{J}(\mathbf{\Omega},\mathbf{d})-\mathcal{J}^*(\mathbf{d})$ for $\mathcal{J}^*$ and $\mathcal{J}$ of~\eqref{eq_Jstar} and~\eqref{eq_stealth_obj}, the optimal value $\mu^*$ of~\eqref{eq_prop_nonconvex} satisfies
\begin{align}
    \label{eq_prop_regret1}
     \regret_{\mathcal{J}}(\mathbf{\Omega}^*,\mathbf{d}) \leq \mu^*\mathrm{,~\forall\alpha\text{-}stealthy~attacks~\mathbf{d}}
\end{align}
and also, for the worst-case $\alpha$-stealthy attack $\mathbf{d_{wc}}(\mathbf{\Omega})$ (\ie{}, the minimizer of~\eqref{eq_stealth_qcqp}, with the optimal value given in Theorem~\ref{thm_regret_metric}), we have
\begin{align}
    \label{eq_prop_regret2}
     \mu^* = \regret_{\mathcal{J}}(\mathbf{\Omega}^*,\mathbf{d}^*) \leq \regret_{\mathcal{J}}(\mathbf{\Omega},\bar{\mathbf{d}})\mathrm{,~\forall\mathbf{\Omega}~with~\eqref{eq_sls_conditions}}~~~
\end{align}
where $\mathbf{d}^* = \mathbf{d_{wc}}(\mathbf{\Omega}^*)$ and $\bar{\mathbf{d}} = \mathbf{d_{wc}}(\mathbf{\Omega})$.
\end{proposition}
\begin{proof}
As discussed in Lemma~\ref{lemma_sls}, the conditions~\eqref{eq_sls1_prop} and~\eqref{eq_sls2_prop} ensures that the feedback controller with $\mathbf{K} = \mathbf{K}^* = \mathbf
{L}^*-\mathbf{M}^*{\mathbf{R}^*}^{-1}\mathbf{N}^*$ achieves the desired response~\eqref{eq_system_with_feedback}. Since the problem~\eqref{eq_prop_nonconvex} is formulated to find $\mathbf{\Omega}$ that minimizes the metric $\mu$ of~\eqref{eq_regret_metric_convex} in Theorem~\ref{thm_regret_metric}, the relations~\eqref{eq_prop_regret1} and~\eqref{eq_prop_regret2} naturally follow by construction of $\varsigma$ in~\eqref{eq_stealth_qcqp}. 
\end{proof}

Thanks to the affine nature of the system level parameterization given in Lemma~\ref{lemma_sls}, the system level constraints $\mathfrak{S}$ can handle a large variety of system properties, including, but limited to, temporal and spatial locality, distributed control, and scalability~\cite{sls_ARC,sls_output_feedback_control,sls_tutorial}. Specifically, for networked control systems, the control gain can be modified by switching the topology as in~\eqref{eq_output_feedback} and we can easily add distributed control constraints \textit{affinely} in terms of the network topology directly in~\eqref{eq_sls_parameterization}. This leads to the following assumption.
\begin{assumption}
\label{assump_affine_sls_topology}
Given the history of topologies of $\bm{\nu}$~\eqref{eq_sls_parameterization} and their adjacency matrices, we can define a convex constraint $\mathbf{\Omega} \in \mathfrak{C}(\bm{\nu})$ for restricting $\mathbf{\Omega}$ to be in a set consistent with the network topologies and the system's causality.
\end{assumption}

However, the optimization problem~\eqref{eq_prop_nonconvex} of Proposition~\ref{proposition_sls_rstealthy_regret} is still nonlinear even with $\mathfrak{S} = \mathfrak{C}(\bm{\nu})$ using Assumption~\ref{assump_affine_sls_topology}. Before proceeding, let us introduce the following lemma useful for convexification (see also, \eg{},~\cite{BoydRankRelaxation,rank_constrained_kyotoU}).
\begin{lemma}
\label{lemma_rank}
For any real column vector $a\in\mathbb{R}^b$ and real symmetric matrix $S\in\mathbb{S}^{b\times b}$, we have the following:
\begin{align}
    \label{eq_rank_equivalence}
    \{(a,S)|S=aa^{\top}\} = \left\{(a,S)\left|\begin{bmatrix}
        S & a \\
        a^{\top} & 1
    \end{bmatrix} \succeq 0~\&~\rank(S)=1\right.\right\}~~~
\end{align}
\end{lemma}
\begin{proof}
Let $\mathrm{(LHS)}=\mathfrak{L}$ and $\mathrm{(RHS)}=\mathfrak{R}$. 

($\mathfrak{L}\subset\mathfrak{R}$): Since $\rank(S) = \rank(aa^{\top}) = 1$ and $S=aa^{\top}\Rightarrow S\succeq aa^{\top}$, applying Schur's complement lemma~\cite[pp. 650-651]{citeulike:163662} shows $\mathfrak{L}\subset\mathfrak{R}$.

($\mathfrak{R}\subset\mathfrak{L}$): Since $S$ is real symmetric, we can always write $S$ as $S = V\diag(\varpi_1,\cdots,\varpi_b)V^{\top}$, where $V$ is an orthogonal matrix of the orthonormal eigenvectors and $\varpi_i$ are the real eignenvalues of $S$. Also, since $\rank(S) = 1$, $S$ has at most one non-zero eigenvalue $\varpi$, which implies $S = \varpi vv^{\top}$ for the corresponding unit eigenvector $v$. Defining $a$ as $a = \sqrt{\varpi} v$ shows $\mathfrak{R}\subset\mathfrak{L}$.
\end{proof}

The following theorem provides one way to reformulate the problem~\eqref{eq_prop_nonconvex} of Proposition~\ref{proposition_sls_rstealthy_regret} into an almost equivalent optimization problem in a computationally efficient form. 
\begin{theorem}
\label{thm_convex_rank_constraint}
Suppose that Assumption~\ref{assump_affine_sls_topology} holds and $\mathfrak{S} = \mathfrak{C}(\bm{\nu})$ in~\eqref{eq_prop_nonconvex}. Consider the following optimization problem, the objective and the constraints of which are all convex except for the rank constraints of~\eqref{eq_con_thmconvexrank4}:
\begin{subequations}
\label{eq_thm_convexrank}
\begin{align}
    &\bar{\mu}^* = \min_{\mathbf{\Omega},\bm{\lambda},\bm{\mathcal{X}},\mathbf{\Lambda}}\lambda\alpha\label{eq_thm_convexrank_obj}\textcolor{white}{\eqref{eq_thm_convexrank_obj}} \\
    &\mathrm{\st{}}~
    \begin{bmatrix}
        \lambda_{\mathrm{inv}}\mathcal{Q}+\ell(\bm{\mathcal{X}}) & \Psi(\mathbf{\Omega})^{\top} \\
        \Psi(\mathbf{\Omega}) & \lambda\mathbb{I}
    \end{bmatrix} \succeq 0,~\eqref{eq_sls1_prop},~\eqref{eq_sls2_prop} \label{eq_con_thmconvexrank1}\textcolor{white}{\eqref{eq_con_thmconvexrank1}} \\
    &\textcolor{white}{\mathrm{\st{}}~}
    \begin{bmatrix}
        \bm{\mathcal{X}} & \matvec(\Phi(\mathbf{\Omega})) \\
        \matvec(\Phi(\mathbf{\Omega}))^{\top} & 1
    \end{bmatrix} \succeq 0,~
    \begin{bmatrix}
        \mathbf{\Lambda} & \bm{\lambda} \\
        \bm{\lambda}^{\top} & 1
    \end{bmatrix} \succeq 0, \label{eq_con_thmconvexrank2}\textcolor{white}{\eqref{eq_con_thmconvexrank2}}\\
    &\textcolor{white}{\mathrm{\st{}}~}\mathbf{\Omega} \in \mathfrak{C}(\bm{\nu}),~\bm{\lambda} = [\lambda,\lambda_{\mathrm{inv}}]^{\top},~\lambda > 0,~\mathbf{\Lambda}_{12} = \mathbf{\Lambda}_{21} = 1 \label{eq_con_thmconvexrank3}\textcolor{white}{\eqref{eq_con_thmconvexrank3}} \\
    &\textcolor{white}{\mathrm{\st{}}~}\rank(\bm{\mathcal{X}}) = 1, \rank(\mathbf{\Lambda}) = 1 \label{eq_con_thmconvexrank4}\textcolor{white}{\eqref{eq_con_thmconvexrank4}}
\end{align}
\end{subequations}
where $\ell$ is a linear function of the decision variable $\bm{\mathcal{X}}$ defined by $\ell(\bm{\mathcal{X}}) = \Phi(\mathbf{\Omega})^{\top}\Phi(\mathbf{\Omega})$, $\matvec(\Phi(\mathbf{\Omega}))$ denotes the vectorization of the matrix $\Phi(\mathbf{\Omega})$, and the other notations are consistent with the ones of Proposition~\ref{proposition_sls_rstealthy_regret}. If $\lambda^* \neq 0$ for the optimizer $(\lambda^*,\Omega^*)$ of~\eqref{eq_prop_nonconvex}, which is the case when the optimal regret $\mu^* = \regret_{\mathcal{J}}(\mathbf{\Omega}^*,\mathbf{d}^*) > 0$ in~\eqref{eq_prop_regret2}, then we have
\begin{align}
    \label{eq_mu_equal}
    \bar{\mu}^* = \mu^*.
\end{align}
If $\lambda^* = 0$, which is the case when the optimal regret $\mu^* = \regret_{\mathcal{J}}(\mathbf{\Omega}^*,\mathbf{d}^*) = 0$, then we have
\begin{align}
    \label{eq_mu_not_equal}
    \bar{\mu}^* \geq \mu^*.
\end{align}
\end{theorem}
\begin{proof}
If $\lambda^* \neq 0$ in~\eqref{eq_prop_nonconvex}, \ie{}, $\mu^* = \regret_{\mathcal{J}}(\mathbf{\Omega}^*,\mathbf{d}^*) > 0$ in~\eqref{eq_prop_regret2}, the constraint~\eqref{eq_con_prop} can be equivalently expressed as
\begin{align}
    &\begin{bmatrix}
        \lambda_{\mathrm{inv}}\mathcal{Q}+\mathcal{P} & \Psi(\mathbf{\Omega})^{\top} \\
        \Psi(\mathbf{\Omega}) & \lambda\mathbb{I} \label{eq_nonlinaer_lmi}
    \end{bmatrix} \succeq 0, \\
    &\lambda \lambda_{\mathrm{inv}} = 1,~\mathcal{P} = \Phi(\mathbf{\Omega})^{\top}\Phi(\mathbf{\Omega}) \label{eq_nonlinaer_quadratic}
\end{align}
using Schur's complement lemma~\cite[pp. 650-651]{citeulike:163662}, which is nonlinear due to the equality constraints~\eqref{eq_nonlinaer_quadratic}. Still, since the nonlinearity is at most quadratic/bilinear, these constraints can be written as a function of additional decision variables (\ie{}, liftings) for $\mathbf{\Lambda} = \bm{\lambda}\bm{\lambda}^{\top}$ and $\bm{\mathcal{X}} = \matvec(\Phi(\mathbf{\Omega}))\matvec(\Phi(\mathbf{\Omega}))^{\top}$, where $\bm{\lambda} = [\lambda,\lambda_{\mathrm{inv}}]^{\top}$. This observation leads to the following equivalent constraints of~\eqref{eq_nonlinaer_quadratic} due to~\eqref{eq_rank_equivalence} of Lemma~\ref{lemma_rank}:
\begin{align}
    \eqref{eq_nonlinaer_quadratic} \Leftrightarrow& 
    \begin{bmatrix}
        \bm{\mathcal{X}} & \matvec(\Phi(\mathbf{\Omega})) \\
        \matvec(\Phi(\mathbf{\Omega}))^{\top} & 1
    \end{bmatrix} \succeq 0,~
    \begin{bmatrix}
        \mathbf{\Lambda} & \bm{\lambda} \\
        \bm{\lambda}^{\top} & 1
    \end{bmatrix} \succeq 0, \\
    \textcolor{white}{\eqref{eq_nonlinaer_quadratic} \Leftrightarrow}&\rank(\bm{\mathcal{X}}) = 1,~\rank(\mathbf{\Lambda}) = 1.
\end{align}
Rewriting the constraints~\eqref{eq_nonlinaer_lmi} and~\eqref{eq_nonlinaer_quadratic} using these additional lifted variables completes the proof for~\eqref{eq_mu_equal}.

The relation~\eqref{eq_mu_not_equal} can be immediately obtained by the fact that $\{\lambda\in\mathbb{R}|\lambda > 0\} \subset \{\lambda\in\mathbb{R}|\lambda \geq 0\}$.
\end{proof}

Since the optimization problem derived in Theorem~\ref{thm_convex_rank_constraint} is convex except for the rank constraint, we can readily apply a large number of convex rank minimization tools available in the literature, including, but not limited to,~\cite{BoydRankRelaxation,rank_constrained_kyotoU,rank_constrained_boyd,rank_constrained_microsoft,rank_constrained_pourdue_ran}.

==> archive/sections/5_extension.tex <==
\section{Extensions}
\label{sec_extension}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
This section discusses several extensions of the topology switching strategy of Proposition~\ref{proposition_sls_rstealthy_regret} and Theorem~\ref{thm_convex_rank_constraint}, which implies broad applicability of our regret optimal metric under stealthy attacks in a wide variety of more general problem settings.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Relaxed Regret Optimal Control}
As in the relaxed, suboptimal $\mathcal{H}_{\infty}$ control (see \eg{},~\cite{256331}), we could also suboptimally consider a bounded regret optimal gain for stealthy attacks in Proposition~\ref{proposition_sls_rstealthy_regret}, instead of optimizing it, which results in a simpler optimization problem as follows.
\begin{corollary}
\label{corollary_suboptimal_hinfinity}
If we consider a relaxed problem with a fixed $\lambda = \bar{\lambda}\in\mathbb{R}_{+}$ in~\eqref{eq_prop_nonconvex} of Proposition~\ref{proposition_sls_rstealthy_regret}, then the problem~\eqref{eq_thm_convexrank} can be simplified to the following feasibility problem as follows:
\begin{subequations}
\label{eq_corollary_convexrank}
\begin{align}
    &\mathrm{Find}~(\mathbf{\Omega},\bm{\mathcal{X}})\label{eq_corollary_convexrank_obj}\textcolor{white}{\eqref{eq_corollary_convexrank_obj}} \\
    &\mathrm{\st{}}~
    \begin{bmatrix}
        \mathcal{Q}+\lambda\ell(\bm{\mathcal{X}}) & \Psi(\mathbf{\Omega})^{\top} \\
        \Psi(\mathbf{\Omega}) & \mathbb{I}
    \end{bmatrix} \succeq 0,~\eqref{eq_sls1_prop},~\eqref{eq_sls2_prop} \label{eq_corollary_convexrank1}\textcolor{white}{\eqref{eq_corollary_convexrank1}} \\
    &\textcolor{white}{\mathrm{\st{}}~}
    \begin{bmatrix}
        \bm{\mathcal{X}} & \matvec(\Phi(\mathbf{\Omega})) \\
        \matvec(\Phi(\mathbf{\Omega}))^{\top} & 1
    \end{bmatrix} \succeq 0,~\mathbf{\Omega} \in \mathfrak{C}(\bm{\nu}),\label{eq_corollary_convexrank2}\textcolor{white}{\eqref{eq_corollary_convexrank2}} \\
    &\textcolor{white}{\mathrm{\st{}}~}\rank(\bm{\mathcal{X}}) = 1 \label{eq_corollary_convexrank3}\textcolor{white}{\eqref{eq_corollary_convexrank3}}
\end{align}
which is convex except for the rank condition~\eqref{eq_corollary_convexrank3}.
\end{subequations}
\end{corollary}
\begin{proof}
This follows from Theorem~\ref{thm_convex_rank_constraint} by fixing $\lambda=\bar{\lambda}$.
\end{proof}

Also, dropping the rank constraints in the problems~\eqref{eq_thm_convexrank} and~\eqref{eq_corollary_convexrank} results in a convex optimization problem with a well-known relaxation approach.
\begin{corollary}
Applying Shor's relaxation~\cite{shor_original} to the problem~\eqref{eq_prop_nonconvex} of Proposition~\ref{proposition_sls_rstealthy_regret} yields the problem~\eqref{eq_thm_convexrank} of Theorem~\ref{thm_convex_rank_constraint} without the rank constraints~\eqref{eq_con_thmconvexrank4}. The solution of this problem $\bar{\mu}^*_{\mathrm{shor}}$ gives the lower bound of $\mu^*$ in~\eqref{eq_obj_prop}, \ie{},
\begin{align}
    \bar{\mu}^*_{\mathrm{shor}} \leq \mu^*.
\end{align}
\end{corollary}
\begin{proof}
This follows from~\eqref{eq_rank_equivalence} of Lemma~\ref{lemma_rank}, which indicates that dropping the rank constraint there results in Shor's relaxation. See also, \eg{}, \cite[pp. 220-225]{Shor1998Book},\cite{BoydRankRelaxation}.
\end{proof}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Sparsity}
If the convex constraint $\mathbf{\Omega} \in \mathfrak{C}(\bm{\nu})$ of~\eqref{eq_con_thmconvexrank3} in Theorem~\ref{thm_regret_metric} includes sparsity constraints due to, \eg{}, distributed communications of the network, we could use the following corollary for additional simplification.
\begin{corollary}
\label{eq_corollary_sparcity}
Suppose that we have sparsity constraints for $\mathbf{\Omega}$, which leads to lienar constraints of the form $\matvec(\mathbf{\Phi}(\mathbf{\Omega}))_i = 0$. Then all the entries in the $i$th column and $i$th row of the matrix $\bm{\mathcal{X}}$ of~\eqref{eq_thm_convexrank} in Theorem~\ref{thm_regret_metric} are also equal to zero.
\end{corollary}
\begin{proof}
This follows from the definition of $\bm{\mathcal{X}}$ introduced in the proof of Thereom~\ref{thm_convex_rank_constraint}.
\end{proof}
Another potential direction for addressing sparsity is considering spatial regret defined as the regret between the cost of a topology $\mathbf{\Omega}$ which belongs to a sparse set $\mathfrak{C}(\bm{\nu})$, and that of a topology $\hat{\mathbf{\Omega}}$ which belongs to a denser set $\mathfrak{C}(\bm{\hat{\nu}})$:

SpRegret($\mathbf{\Omega}$,$\hat{\mathbf{\Omega}}$)= $\max_{\|d\| \leq 1} J(\mathbf{\Omega},d)-J(\hat{\mathbf{\Omega}},d)$.

Under no further constraints, ideally, the constraint set should be quadratically invariant (QI) w.r.t $XX$ to ensure optimality of the the control strategy. In cases where it is not, there are methods that allow for the synthesis of the controller even when the set isn't QI. Here, we use the denser topology as the one that satisfies QI condition, closing thus the QI optimality gap.

We could further extend the notion of regret to SpatioTemporalRegret by defining it as the difference in costs of a sparse topology and of a denser topology that also knows the future attacks. In this case, the challenge we face is ensuring that the problem is well-posed (regret>0), and finding the closest QI, noncausal sparse set...
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Controllability, Observability, Detectability}
As discussed in~\eqref{}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Additional Constraints and Locality}
We can clearly see that the control input $\mathbf{u}$ in~\eqref{eq_sls_parameterization} of Sec.~\ref{sec_sls} is linear in the system level parameters $\mathbf{\Omega}$, the constraint
\begin{align}
    \|\mathbf{u}\| = \|\mathbf{M}\mathbf{d_x}+\mathbf{D}\mathbf{d_y}\|_* \leq u_{\max}
\end{align}
where $u_{\max}\in\mathbb{R}_{+}$ is some constant, is always a convex constraint for any norm $*$. We can also consider other performance requirements as convex constraints on top of the problems~\eqref{eq_thm_convexrank} of Theorem~\ref{thm_convex_rank_constraint} and~\eqref{eq_corollary_convexrank} of Corollary~\ref{eq_corollary_convexrank}, the examples of which are given in~\cite{sls_ARC,sls_tutorial,sls_output_feedback_control}.

For large-scale networks, we could apply spatiotemporal constraints to further reduce the computational burden thanks to the system level parameterization. In particular, if we assume that 1) the closed-loop disturbance responses have finite-impulse responses and that 2) the effects of disturbances are felt only in local neighborhoods of each agent, then we can decompose the problems~\eqref{eq_thm_convexrank} of Theorem~\ref{thm_convex_rank_constraint} into small subproblems that can be solved locally~\cite{sls_ARC,sls_tutorial,sls_output_feedback_control}. This allows model predictive control-like formulation of the system level synthesis~\cite{slsmpc}.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Data-Driven Control and Robustness}
The system level parameterization is also useful for the case where we have access only to the system's input and output data $u_{[0,T_\mathrm{data}-1]} = \{u_0,\cdots,u_{T_\mathrm{data}-1}\}$ and $y_{[0,T_\mathrm{data}-1]} = \{y_0,\cdots,y_{T_\mathrm{data}-1}\}$ of the system~\eqref{eq_system} with $a_k=0$. Let $\mathcal{H}(\sigma_{[0,j]})$ be the Hankel matrix of depth $D$, associated with the signal $\sigma_{[0,T_{\mathrm{data}}-1]}$ defined as follows:
\begin{align}
    \label{eq_Hankel}
    \mathcal{H}(\sigma_{[0,T_{\mathrm{data}}-1]}) = 
    \begin{bmatrix}
        \sigma_0 & \cdots & \sigma_{T_{\mathrm{data}}-D} \\
        \vdots & \ddots & \vdots \\
        \sigma_{D-1} & \cdots & \sigma_{T_{\mathrm{data}}-1}
    \end{bmatrix}
\end{align}
where $D \leq T_{\mathrm{data}}$.
\begin{definition}
\label{def_persistently_exciting}
The signal $\sigma_{[0,T_{\mathrm{data}}-1]}$ is persistently exciting of order $D$ if the Hankel matrix $\mathcal{H}(\sigma_{[0,T_{\mathrm{data}}-1]})$~\eqref{eq_Hankel} has full row rank.
\end{definition}

The Hankel matrix of~\eqref{eq_Hankel} leads to the following lemma essential in the data-driven system level synthesis~\cite{Willems_fundamental,Willems_fundamental_state_space}.
\begin{lemma}
\label{lemma_Willems}
Suppose that the input data $u_{[0,T_\mathrm{data}-1]}$ is persistently exciting of order $n+D$ as in Definition~\ref{def_persistently_exciting}, where $n$ is the number of the system state $x$ of~\eqref{eq_continuous_initialx}. Then $(\bar{u}_{[0,D-1]},\bar{y}_{[0,D-1]})$ is a valid input/output trajectory of~\eqref{eq_system} with $a_k = 0$ if and only if $\exists g\in\mathbb{R}^{T_\mathrm{data}-D+1}$ \st{}
\begin{align}
    \label{eq_Williems}
    \begin{bmatrix}
        u_{[0,T_\mathrm{data}-1]} \\
        y_{[0,T_\mathrm{data}-1]}
    \end{bmatrix}
    =
    \begin{bmatrix}
        \mathcal{H}(u_{[0,T_{\mathrm{data}}-1]}) \\
        \mathcal{H}(y_{[0,T_{\mathrm{data}}-1]})
    \end{bmatrix}g.
\end{align}
\end{lemma}
\begin{proof}
    See,~\eg{},~\cite{Willems_fundamental,Willems_fundamental_state_space}.
\end{proof}

It is shown in~\cite{data_driven_sls} that $g$ of~\eqref{eq_Williems} in Lemma~\ref{lemma_Willems} can be characterized by the system level parameterization of~\eqref{eq_sls_parameterization} for the case of full-state feedback. Its robust properties allow for extending this idea to perturbed trajectory data as also shown in~\cite{data_driven_sls}. These observations imply the great potential of our approach to model-free settings as in~\cite{data_driven_sls,data_sls_mpc,sls_data_predictive}.

